Multi-View Surveillance Video Summarization via Joint Embedding and Sparse Optimization

Most traditional video summarization methods are designed to generate effective summaries for single-view videos, and thus they cannot fully exploit the complicated intra and inter-view correlations in summarizing multi-view videos in a camera network. In this paper, with the aim of summarizing multi-view videos, we introduce a novel unsupervised framework via joint embedding and sparse representative selection. The objective function is two-fold. The first is to capture the multi-view correlations via an embedding, which helps in extracting a diverse set of representatives. The second is to use a `2;1- norm to model the sparsity while selecting representative shots for the summary. We propose to jointly optimize both of the objectives, such that embedding can not only characterize the correlations, but also indicate the requirements of sparse representative selection. We present an efficient alternating algorithm based on half-quadratic minimization to solve the proposed non-smooth and non-convex objective with convergence analysis. A key advantage of the proposed approach with respect to the state-of-the-art is that it can summarize multi-view videos without assuming any prior correspondences/alignment between them, e.g., uncalibrated camera networks. Rigorous experiments on several multi-view datasets demonstrate that our approach clearly outperforms the state-of-the-art methods.

==> Discussions.tex <==
\underline{\textit{Interestingness of Video Shots:}} As existing approaches, we compute the shot interestingness score by taking into account the rest of the video shots. Specifically, we first compute the shot interestingness score as the sum of scores predicted for each frame that belong to the shot and then take the relative score over the maximum predicted score in a video. We follow~\cite{LucVanGool2014} to compute the interestingness score of each frame by considering attention, asthetic quality and presence of landmarks/persons. Note that these forms of interestingness prediction are often used in several vision tasks and are quite flexible~\cite{Graumann2012,ejaz2013efficient,datta2006studying,dhar2011high,smith1997video}. However, one can also learn a regression model to predict an interestingness score of domain relevance~\cite{gygli2015video,Ranking2014,yaohighlight} or compute with user specifications via human in the loop~\cite{han2011personalized} - we expect more sophisticated ones will only benefit our proposed approach. Concretely speaking, our method is not dependent on a particular definition on interestingness. 


\vspace{1mm}
\underline{\textit{Correlation between Video Shots:}} There are a lot of ways to measure the correlation between two shots ${{c_{\it{ij}}}}$. In this paper, we employ Scott and Longuet-Higgins (SLH) algorithm~\cite{Scott1991} with Gaussian kernel to measure the correlation, since it is simple to implement and it performs well in several vision tasks~\cite{permutation2013,torki2010one}.
Specifically, given the shot feature similarity matrix ${S}$, computed via a Gaussian kernel between two videos, SLH algorithm finds an orthonormal matrix ${C}$ that permutes the rows of $S$ in order to maximize its trace. Mathematically,
\vspace{-1mm}
\begin{equation}
\begin{gathered}
\label{eq:SLH}
{C} = \argmax_{{C}^T {C}=I} \  tr({C}^T {S})
\end{gathered}
\vspace{-1mm}
\end{equation} 
Maximizing the above function is a singular value decomposition problem and the optimal solution is given by ${C}^{*} = {U}{D}{V}^T$, where the SVD decomposition of ${S}={U}{E}{U}^T$ and ${D}$ is obtained by replacing singular values of ${E}$ by ones. We use the matrix ${C}^{*}$ as the correlation matrix after setting the negative values to 0~\cite{torki2010one}. 
We will discuss the peformance benefits in employing such correlations compared to the cosine similairy in the experiments. It is also important to mention here that our proposed formulation (\ref{eq:multivideo}) is highly flexible to incorporate any type of correlations defined between two shots.       

\vspace{1mm}
\underline{\textit{Sparsity Regularization Parameter:}} The regularization parameter $\lambda$ in (\ref{eq:onevfinal3}) puts a trade-off between two opposing terms: the reconstruction error and number of representative shots. In other words, we obtain a small reconstruction error by selecting more representative shots and vice versa. As indicated by the update equation of $Z$ in Algo.~\ref{algo:ADMM}, when $\lambda$ is large enough, e.g., $\lambda \geq \lambda^{max}$, we get $Z=0$ that means we select no representaive shots. 
Thus, to avoid an empty selection, we let $\lambda \leq \lambda^{max}$ and obtain $\lambda^{max}= \max_{0 \leq i \leq n} ||x_i^{T}X||_2$, as in~\cite{Ehsan2012}.
In our experiments, we let $\lambda=\frac{\lambda^{max}}{\alpha}$ and tune $\alpha$ between the interval [2,30]~\cite{Ehsan2012}. A smaller $\alpha$ indicates a sparser solution.
%\vspace{1mm}
%\underline{\textit{Matrix Inverse in Algo.~\ref{algo:ADMM}:}} We do not require to compute $({X}^{T}{X}+\mu{I})^{-1}$ in each iteration for updating ${U}$. More specifically, it is unchanged during iterations of Algo.~\ref{algo:ADMM}. Thus, we pre-compute the required Cholesky factorizations to avoid redundant computations for efficiently solving those linear systems. 
%Moreover, for very large problems, Sherman-Morrison-Woodbury formula can also be employed to transform it to a smaller $m\times m$ linear system.

\vspace{1mm}
\underline{\textit{Intialization in Algo.~\ref{algo:OverallALM}:}} Since the alternating minimization can make the Algo.\ref{algo:OverallALM} stuck in a local minimum, it is important to have a sensible initialization.
We initialize the sparse coefficient matrices of $m-1$ videos by solving (\ref{eq:naivemultivideo}) using Algo.~\ref{algo:ADMM}, which is a special case (when $\lambda_d = 0$ in (\ref{eq:multivideo})) of our method. After the initialization, the follwoing question remain: from which view we should start the alternating minimization? One possible way is to randomly start with any video and repeat the minimization over all videos until convergence. However, since we have some prior knoweldge on which video is more informative in the collection, we can start with initializing and fixing more informative videos, and optimize with respect to the least informative video. More specifically, we start with the specific ${{Z^{(\it{v})}}}$ which has more number of nonzero rows after solving (\ref{eq:naivemultivideo}) since the number of nonzero rows indicate the relative importance of each video in the collection.

\vspace{1mm}
\underline{\textit{Stopping Criteria:}} In Algo.~\ref{algo:ADMM}, the stop criteria is set to $||U^{(t)}-Z^{(t)}||_{\infty} \leq \epsilon  \ or \ t \geq 2000$, where $t$ is the iteration number and $\epsilon$ is set to $10^{-7}$ throughout the experiments. Similarly, in Algo.~\ref{algo:OverallALM}, we set the stop criteria as $\frac{|f^{(t+1)}-f^{(t)}|}{f^{(t)}}<10^{-2}$, where ${f^{(t)}}$ is the objective value in the $t$-th iteration.

\vspace{1mm}
\underline{\textit{Convergence Analysis:}} We can prove the convergence of the proposed Algo.~\ref{algo:OverallALM} as follows: we divide the problem (\ref{eq:multivideo}) into $m$ number of subproblems and each of them is a convex problem with respect to one variable (Algo.~\ref{algo:ADMM}). The convergence of Algo.~\ref{algo:ADMM} is guaranteed by the existing ADMM theory~\cite{glowinski1989augmented}. Therefore, by solving the subproblems alteranatively, our proposed algorithm will guarantee that we can find the optimal solution to each subproblem and finally, the algorithm will converge to the local solution. 
%In practice, we monitor the convergence by the relative difference in the value of the objective between two consecutive iterations, and stop when the difference falls below a minimum threshold of $10^{-2}$. 
In all our experiments, we monitor the convergence is reached within less than 10 iterations.

\vspace{1mm}
\underline{\textit{Time Complexity Analysis:}} 
%Our proposed approach results in a computational time complexity which are of the order of the problem size. Furthemore, it allows for parallel implementation, which can further reduce the computational time. 
As discussed earlier, our overall problem can be divided into $m$ number of subproblems and each of them can be solved using Algo.~\ref{algo:ADMM}, we first analyze the computational complexity of Algo.~\ref{algo:ADMM} and then present the total complexity of our method. We also show that the proposed approach allows for parallel implementation, which can further reduce the computational time to a large extent. 

In Algo.~\ref{algo:ADMM}, each iteration contains three substeps (See Appendix for details):
(i) solving a linear system with respect to $U$ for once and is not repeated for each iteration. Solving this requires at most complexity of $\mathcal{O}(n_v^{3})$. However, we can solve this via $n_v$ indepedent smaller linear systems over the $n_v$ columns of $U$. Thus, with $P$ parallel processing resources, we can reduce the computational time to $\mathcal{O}(n_v^{3}/P)$,
(ii) update with respect to $Z$ can be done in $\mathcal{O}(n_v^{2})$ computational time. However, since the solution correspond to one-dimensional shrinkage and thresholding operation, we can perform the update via $n_v$ indepedent shrinkage operations over the $n_v$ rows of $Z$. Thus, with $P$ parallel processing resources, this can be reduced to $\mathcal{O}(n_v^{2}/P)$,
(iii) similarly, update on $\Lambda$ can be done in $\mathcal{O}(n_v^{2}/P)$ computational time with $P$ parallel processing resources by performing $n_v$ indepedent updates over rows or columns. As a result, the computational complexity of Algo.~\ref{algo:ADMM} is $\mathcal{O}(n_v^{3}+2*n_v^{2}) \approx \mathcal{O}(n_v^{3})$ and it reduces to $\mathcal{O}(n_v^{3}/P)$ with $P$ parallel processing resources. The proposed approach invokes Algo.~\ref{algo:ADMM} for each subproblem i.e., with respect to one video alternatively. By adopting the same procedure, the computational complexity of our approach is $\mathcal{O}(\sum_{v=1}^{m}{n_v^{3}})$. Note that time complexity for solving a linear system can be reduced from $\mathcal{O}(n_v^{3})$ to $\mathcal{O}(n_v^{2.376})$ using the Coppersmith-Winograd algorithm. Therefore, the time complexity of our approach is $\mathcal{O}(\sum_{v=1}^{m}{n_v^{2.376}})$ and it reduces to $\mathcal{O}([\sum_{v=1}^{m}{n_v^{2.376}}]/P)$ with $P$ parallel processing resources.   





==> MathDetails.tex <==
\begin{equation}
	\begin{gathered}
		\label{eq:singlevideo}
		\min_{\bf{Z^{(\it{v})}}}\ \lVert {\bf{X^{\it{(v)}}} - \bf{X^{\it{(v)}}Z^{\it{(v)}}} \rVert}^2_{F} + \lambda^{\it{(v)}}_s\lVert {\bf{Z^{\it{(v)}}}\rVert}_{2,1} \\
		s.t.\ \ {\bf{Z^{(\it{v})^{T}}}1 = 1},\ {\bf{Z^{(\it{v})}}} \in \mathbb{R}^{n_v\times n_v}
	\end{gathered}
%	\vspace{-2mm}
\end{equation}  

\begin{equation}
\begin{gathered}
\label{eq:naivemultivideo}
\min_{\bf{Z^{(1)}},\bf{Z^{(2)}},\cdots,\bm{Z^{({m})}}} \ \sum_{v=1}^{m}\lVert {\bf{X^{\it{(v)}}} - \bf{X^{\it{(v)}}Z^{\it{(v)}}} \rVert}^2_{F} + \sum_{v=1}^{m} \lambda^{\it{(v)}}_s\lVert {\bf{Z^{\it{(v)}}}\rVert}_{2,1} \\
s.t.\ \ {\bf{Z^{(\it{v})^{T}}}1 = 1},\ {\bf{Z^{(\it{v})}}} \in \mathbb{R}^{n_v\times n_v},\ \forall \ 1 \leq \it{v} \leq m	
\end{gathered}
%	\vspace{-2mm}
\end{equation}

\begin{equation}
\begin{gathered}
\label{eq:diversity}
{f_{d}({\bf{Z^{(\it{v})}}},\bf{Z^{(\it{w})}})} = \frac{1}{\it{n}_{v}n_{w}}\sum_{i=1}^{n_v}\sum_{j=1}^{n_w}\lVert{\bf{Z^{(\it{v})}_{\it{i}}} \rVert}_{2,1}{\bf{C_{\it{ij}}}}\lVert{\bf{Z^{(\it{w})}_{\it{j}}} \rVert}_{2,1}
\end{gathered}
%\vspace{-2mm}
\end{equation}

\begin{equation}
\begin{gathered}
\label{eq:diversityW}
{\bf{W^{\it{(vw)}}_{\it{ii}}}} = \frac{1}{\it{n}_{v}n_{w}}\sum_{j=1}^{n_w}{\bf{C_{\it{ij}}}}\lVert{\bf{Z^{(\it{w})}_{\it{j}}} \rVert}_{2,1}
\end{gathered}
%\vspace{-2mm}
\end{equation} 

\begin{equation}
\begin{gathered}
\label{eq:diversityfinal}
{f_{d}({\bf{Z^{(\it{v})}}},\bf{Z^{(\it{w})}})} = \sum_{i=1}^{n_v}\sum_{j=1}^{n_w}\lVert{\bf{Z^{(\it{v})}_{\it{i}}} \rVert}_{2,1}{\bf{C_{\it{ij}}}}\lVert{\bf{Z^{(\it{w})}_{\it{j}}} \rVert}_{2,1}=\lVert{\bf{W^{\it{(vw)}}}\bf{Z^{(\it{v})}} \rVert}_{2,1}
\end{gathered}
%\vspace{-2mm}
\end{equation}   

\begin{equation}
\begin{gathered}
\label{eq:multivideo}
\min_{\bf{Z^{(1)}},\bf{Z^{(2)}},\cdots,\bm{Z^{({m})}}} \underbrace{\sum_{v=1}^{m}\lVert {\bf{X^{\it{(v)}}} - \bf{X^{\it{(v)}}Z^{\it{(v)}}} \rVert}^2_{F}}_{Reconstruction \ error} + \underbrace{\lambda_s \sum_{v=1}^{m} \lVert {\bf{Z^{\it{(v)}}}\rVert}_{2,1}}_{Sparsity} \\ + \underbrace{\lambda_v \sum_{\substack{1\leq v,w\leq m \\ v \neq w}}f_{d}({\bf{Z^{(\it{v})}}},\bf{Z^{(\it{w})}})}_{Diversity} \\  
s.t.\ \ {\bf{Z^{(\it{v})^{T}}}1 = 1},\ {\bf{Z^{(\it{v})}}} \in \mathbb{R}^{n_v\times n_v},\ \forall \ 1 \leq \it{v} \leq m	
\end{gathered}
%	\vspace{-2mm}
\end{equation}   

\begin{equation}
\begin{gathered}
\label{eq:multivideowithonev}
\min_{\bf{Z^{(\it{v})}}}\ \lVert {\bf{X^{\it{(v)}}} - \bf{X^{\it{(v)}}Z^{\it{(v)}}} \rVert}^2_{F} + \lambda_s \lVert {\bf{Z^{\it{(v)}}}\rVert}_{2,1} + \lambda_v \sum_{w=1, v \neq w}^{m}f_{d}({\bf{Z^{(\it{v})}}},\bf{Z^{(\it{w})}}) \\  
s.t.\ \ {\bf{Z^{(\it{v})^{T}}}1 = 1}
\end{gathered}
%	\vspace{-2mm}
\end{equation} 

\begin{equation}
\begin{gathered}
\label{eq:diversityall}
\sum_{w=1, v \neq w}^{m}f_{d}({\bf{Z^{(\it{v})}}},\bf{Z^{(\it{w})}})=\sum_{w=1, v \neq w}^{m}\lVert{\bf{W^{\it{(vw)}}}\bf{Z^{(\it{v})}} \rVert}_{2,1} \\ =\lVert{\bf{W^{\it{(v)}}}\bf{Z^{(\it{v})}} \rVert}_{2,1}
\end{gathered}
%	\vspace{-2mm}
\end{equation} 

\begin{equation}
\begin{gathered}
\label{eq:onev1}
\min_{\bf{Z^{(\it{v})}}}\ \lVert {\bf{X^{\it{(v)}}} - \bf{X^{\it{(v)}}Z^{\it{(v)}}} \rVert}^2_{F} + \lambda_s \lVert {\bf{Z^{\it{(v)}}}\rVert}_{2,1} + \lambda_v \lVert{\bf{W^{\it{(v)}}}\bf{Z^{(\it{v})}} \rVert}_{2,1} \\  
s.t.\ \ {\bf{Z^{(\it{v})^{T}}}1 = 1}
\end{gathered}
%	\vspace{-2mm}
\end{equation} 

\begin{equation}
\begin{gathered}
\label{eq:onev2}
\min_{\bf{Z^{(\it{v})}}}\ \lVert {\bf{X^{\it{(v)}}} - \bf{X^{\it{(v)}}Z^{\it{(v)}}} \rVert}^2_{F} + \lambda \lVert {(\bf{I+W^{\it{(v)}}})\bf{Z^{\it{(v)}}}\rVert}_{2,1} \\  
s.t.\ \ {\bf{Z^{(\it{v})^{T}}}1 = 1}
\end{gathered}
%	\vspace{-2mm}
\end{equation} 

\begin{equation}
\begin{gathered}
\label{eq:onev3}
\min_{\bf{Z^{(\it{v})}}}\ \lVert {\bf{X^{\it{(v)}}} - \bf{X^{\it{(v)}}Z^{\it{(v)}}} \rVert}^2_{F} + \lambda \lVert {\bf{K^{\it{(v)}}}\bf{Z^{\it{(v)}}}\rVert}_{2,1} \\  
s.t.\ \ {\bf{Z^{(\it{v})^{T}}}1 = 1}	
\end{gathered}
%	\vspace{-2mm}
\end{equation}

\begin{equation}
\begin{gathered}
\label{eq:onevfinal}
\min_{\bf{Z^{(\it{v})}}}\ \lVert {\bf{X^{\it{(v)}}} - \bf{X^{\it{(v)}}Z^{\it{(v)}}} \rVert}^2_{F} + \lambda \lVert {\bf{Z^{\it{(v)}}}\rVert}_{\textbf{K},2,1} \\  
s.t.\ \ {\bf{Z^{(\it{v})^{T}}}1 = 1}	
\end{gathered}
%	\vspace{-2mm}
\end{equation}

\begin{equation}
\begin{gathered}
\label{eq:onevfinal2}
\min_{\bf{Z}}\ \lVert {\bf{X} - \bf{X}Z \rVert}^2_{F} + \lambda \lVert {\bf{Z}\rVert}_{\textbf{K},2,1} \\  
s.t.\ \ {\bf{Z^{(\it{v})^{T}}}1 = 1}
\end{gathered}
%	\vspace{-2mm}
\end{equation}

\begin{equation}
\begin{gathered}
\label{eq:onevfinal3}
\underline{\min_{\bf{Z}}\ \lVert {\bf{X} - \bf{X}Z \rVert}^2_{F} + \lambda \lVert {\bf{Z}\rVert}_{\textbf{K},2,1}}
\end{gathered}
%	\vspace{-2mm}
\end{equation}

\begin{equation}
\begin{gathered}
\label{eq:onevfinal4}
\lVert {\bf{X} - \bf{XZ} \rVert}^2_{F}={\lVert {\bf{X}_{\it{original}}} - \bf{X}_{\it{original}}Z \rVert}^2_{F}+\alpha {\lVert \bf{1^{\it{T}}}-\bf{1^{\it{T}}}\bf{Z} \rVert}^2_{F}
\end{gathered}
%	\vspace{-2mm}
\end{equation}

\begin{equation}
\begin{gathered}
\label{eq:admm1}
\min_{\bf{Z,U}}\ \lVert {\bf{X} - \bf{X}U \rVert}^2_{F} + \lambda \lVert {\bf{Z}\rVert}_{\textbf{K},2,1} \\  
s.t.\ \ {\bf{U=Z}}	
\end{gathered}
%	\vspace{-2mm}
\end{equation}

\begin{equation}
\begin{gathered}
\label{eq:admm2}
{\mathcal{L}_{\mu}(\bf{U,Z,\Lambda})} = \frac{1}{2}\lVert {\bf{X} - \bf{XU} \rVert}^2_{F}+\lambda {\lVert \bf{Z} \rVert}_{\textbf{K},2,1}	+ \langle\mathbf{\Lambda}, \textbf{U}-\textbf{Z}\rangle \\ + \dfrac{\mu}{2}\lVert {\textbf{U} - \textbf{Z} \rVert}^2_{F}
\end{gathered}
%	\vspace{-2mm}
\end{equation}

\begin{equation}
\begin{gathered}
\label{eq:admm3}
\min_{\textbf{U}} \ \frac{1}{2}\lVert {\bf{X} - \bf{XU} \rVert}^2_{F}+\langle\mathbf{\Lambda}, \textbf{U}-\textbf{Z}\rangle + \dfrac{\mu}{2}\lVert {\textbf{U} - \textbf{Z} \rVert}^2_{F} \\
\Leftrightarrow \min_{\textbf{U}} \ \frac{1}{2}\textbf{U}^{T}(\textbf{X}^{T}\textbf{X}+\mu\textbf{I})\textbf{U}-(\textbf{X}^{T}\textbf{X}+\mu\textbf{Z}-\mathbf{\Lambda})^{T}\textbf{U}
\end{gathered}
%	\vspace{-2mm}
\end{equation}

\begin{equation}
\begin{gathered}
\label{eq:admm4}
(\textbf{X}^{T}\textbf{X}+\mu\textbf{I})\textbf{U}=(\textbf{X}^{T}\textbf{X}+\mu\textbf{Z}-\mathbf{\Lambda})
\end{gathered}
%	\vspace{-2mm}
\end{equation}

\begin{equation}
\begin{gathered}
\label{eq:admm5}
\underline{\textbf{U}=(\textbf{X}^{T}\textbf{X}+\mu\textbf{I})^{-1}(\textbf{X}^{T}\textbf{X}+\mu\textbf{Z}-\mathbf{\Lambda})}
\end{gathered}
%	\vspace{-2mm}
\end{equation}

\begin{equation}
\begin{gathered}
\label{eq:admm6}
\min_{\textbf{Z}} \ \lambda \lVert {\bf{Z}\rVert}_{\textbf{K},2,1}+\langle\mathbf{\Lambda}, \textbf{U}-\textbf{Z}\rangle+\dfrac{\mu}{2}\lVert {\textbf{U} - \textbf{Z} \rVert}^2_{F}
\end{gathered}
%	\vspace{-2mm}
\end{equation}

\begin{equation}
\begin{gathered}
\label{eq:admm7}
\min_{\textbf{Z}} \ \lambda \lVert {\bf{Z}\rVert}_{\textbf{K},2,1} + \dfrac{\mu}{2}\lVert {\textbf{U} - \textbf{Z}+\mathbf{\Lambda}/\mu \rVert}^2_{F}
\end{gathered}
%	\vspace{-2mm}
\end{equation}

\begin{equation}
\begin{gathered}
\label{eq:admm8}
\min_{\textbf{Z}} \ \sum_{i=1}^{n}\Big [\lambda \textbf{K}_{ii}{\lVert \textbf{Z}_i\rVert}_2+\frac{\mu}{2} {\lVert\textbf{U}_i-\textbf{Z}_i+\frac{1}{\mu}\mathbf{\Lambda}_i \rVert}^2_{F}\Big]
\end{gathered}
%	\vspace{-2mm}
\end{equation}

\begin{equation}
\begin{gathered}
\label{eq:admm9}
\textbf{Z}_i=\max  \Big\{{\lVert r_i \rVert}_2 - \frac{\lambda\textbf{K}_{ii}}{\mu},0\Big\}\frac{r_i}{{\lVert r_i \rVert}_2}
\end{gathered}
%	\vspace{-2mm}
\end{equation}

\begin{equation}
\begin{gathered}
\label{eq:admm10}
\underline{\textbf{Z}=Shrink\Big(\textbf{U}+\frac{\mathbf{\Lambda}}{\mu},\frac{\lambda\textbf{K}}{\mu}\Big)= S_{\frac{\lambda\textbf{K}}{\mu}}(\textbf{U}+\mathbf{\Lambda}/\mu)}
\end{gathered}
%	\vspace{-2mm}
\end{equation}

\begin{equation}
\begin{gathered}
\label{eq:admm12}
\underline{\mathbf{\Lambda} \leftarrow \mathbf{\Lambda} + \mu(\textbf{U-Z})}
\end{gathered}
\end{equation}


\begin{equation}
\begin{gathered}
\label{eq:admm13}
(\textbf{X}^{T}\textbf{X}+\mu\textbf{I})^{-1}=\frac{1}{\mu}\textbf{I}-\frac{1}{\mu}\textbf{X}^{T}(\mu\textbf{I}+\textbf{X}\textbf{X}^{T})^{-1}\textbf{X} \\
(\text{Sherman-Morrison-Woodbury formula})
\end{gathered}
\end{equation}


\begin{algorithm} 
	\caption{An ADMM solver for (\ref{eq:onevfinal3})}\label{algo:ADMM}
	\begin{algorithmic}
		\State {\bf Input:} Video feature matrix $\textbf{X}$, $\textbf{K}$ and $\lambda, \mu >0$  
		\While{\textit{not converged}} \\
		\ \ $\textbf{U} \leftarrow (\textbf{X}^{T}\textbf{X}+\mu\textbf{I})^{-1}(\textbf{X}^{T}\textbf{X}+\mu\textbf{Z}-\mathbf{\Lambda})$;\\
		\ \ $\textbf{Z} \leftarrow S_{\frac{\lambda\textbf{K}}{\mu}}(\textbf{U}+\mathbf{\Lambda}/\mu)$ (row-wise);\\
		\ \ $\mathbf{\Lambda} \leftarrow \mathbf{\Lambda} + \mu(\textbf{U-Z})$;
		\EndWhile
		\State {\bf Output:} Sparse coefficient matrix $\textbf{Z}$.
	\end{algorithmic}
\end{algorithm}

%Since the above algorithm computes the exact solutions for each subproblems, its convergence is guaranteed by the existing ADMM theory under mild conditions, following~\cite{glowinski1989augmented}.
%
%{\bf Theorem 1.} \textit{For $\lambda>0$ and $\mu \in (0,\frac{\sqrt{5}+1}{2})$, the sequence generated $(\textbf{U}_{(k)},\textbf{Z}_{(k)})$ by Algo.~\ref{algo:ADMM} from any starting point $(\textbf{U}_{(0)},\textbf{Z}_{(0)})$ monotonically decreases the objective function value and converges to $(\textbf{U}_{(\star)},\textbf{Z}_{(\star)})$, where $(\textbf{U}_{(\star)},\textbf{Z}_{(\star)})$ is a solution of (\ref{eq:onevfinal3}) and $k$ denotes the iteration number}. 

\begin{algorithm} 
	\caption{Algorithm for solving (\ref{eq:multivideo})}\label{algo:OverallALM}
	\begin{algorithmic}
		\State {\bf Input:} Video feature matrices ${\bf{X^{(1)}},\bf{X^{(2)}},\cdots,\bm{X^{({m})}}}$ 
		\For{\textit{each v}} \\
		\ \ Initialize ${\bf{Z^{(\it{v})}}}$ by solving (\ref{eq:naivemultivideo});
		\EndFor
		\While{\textit{not converged}} 
		\ \ \For{\textit{each v}} \\
			\ \ \ \ \ \ \  Obtain ${\bf{Z^{(\it{v})}}}$ by solving (\ref{eq:onevfinal3}); 
		\EndFor
		\EndWhile
		\State {\bf Output:} Coefficient matrices ${\bf{Z^{(1)}},\bf{Z^{(2)}},\cdots,\bm{Z^{({m})}}}$.
	\end{algorithmic}
\end{algorithm}

%{\bf Theorem 2.} \textit{The alternating optimization procedure in solving (\ref{eq:multivideo}) will monotonically decrease the function value and hence guaranteed to converge with Algo.~\ref{algo:OverallALM}.}
%\newline
%\textbf{Proof.}     


  
    



==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex, bare_jrnl.tex,
                   bare_jrnl_comsoc.tex, bare_jrnl_compsoc.tex,
                   bare_jrnl_transmag.tex
***************************************************************************

